Episodic Learning for Safe Bipedal Locomotion with Control Barrier Functions and Projection-to-State Safety

This paper combines episodic learning and control barrier functions in the setting of bipedal locomotion. The safety guarantees that control barrier functions provide are only valid with perfect model knowledge; however, this assumption cannot be met on hardware platforms. To address this, we utilize the notion of projection-to-state safety paired with a machine learning framework in an attempt to learn the model uncertainty as it affects the barrier functions. The proposed approach is demonstrated both in simulation and on hardware for the AMBER-3M bipedal robot in the context of the stepping-stone problem, which requires precise foot placement while walking dynamically.

==> sections/Amodel.tex <==
\section{Hybrid motion planning}

\begin{figure}[!t]
	\begin{center}
	\vspace{3mm}
		\includegraphics[width=0.43\columnwidth]{Figures/Vision/V35_2.png}
		\includegraphics[width=0.46\columnwidth]{Figures/Vision/model.png}
		\caption{On the left is the rendering of the robot design, and on the right is the illustration of the configuration coordinates for the robot. The leg indices $\mathrm{l}_*$ are shown on the vertices of the \textit{body} link. Each leg has three actuated joints and equipped with a point foot.}
		\label{fig:config}
	\end{center}
	\vspace{-5mm}
\end{figure}

We consider the nonlinear model of quadrupedal locomotion as a hybrid dynamical system, which is an alternating sequence of continuous- and discrete-time dynamics. The order of the sequence is dictated by contact events. In comparison with bipedal walking, the increased number of contact points of quadrupeds increased the complexity of the hybrid model substantially. In this section, we introduce a unified model for quadrupedal behaviors including walking, ambling and trotting, based on which we design full model based optimal controllers as well as simulation validation.

% It is worth noting that this dynamical model is created for model based control purposes, as well as simulation validation.
% Along the course, a series of quadruped behaviors such as walking, ambling and trotting will be introduced. This dynamical model is not only used for simulation validation, but also designed to construct full-model based controllers. synthesized by optimization problems. 

\subsection{The robot}
The robot we study in this paper is the Vision 60-v3.2 (see \figref{fig:robot}), a quadrupedal robot built by Ghost Robotics, with the total weight of $26$ kg and maximum standing height of $0.5$ m. As shown in \figref{fig:config}, we model the quadruped as a $13$-link system: a \textit{body} link and four legs, each of which has three children links ---the \textit{hip}, \textit{upper} and \textit{lower} links. The configuration variables of Vision 60 are denoted by $q\in\mathcal{Q}\subset\R^n$ where $n=18$ is the total number of degrees of freedom (DOF) without considering any contact constraints. Utilizing the floating base convention \cite{Grizzle2014Models}, we can have $q^T =( q_b^T, q_l^T )$, in which $q_b\in\R^3\times\mathrm{SO}(3)$ represents the global Cartesian position and orientation of a frame attached to the \textit{body} linkage, and the local coordinates $q_l\in\R^{12}$ denote the $12$ joint variables: hip roll, hip pitch and knee angles. These angles are denoted by $\theta_{hr_j}, \theta_{hp_j}, \theta_{k_j}$ for the $j$-th leg, all of which are actuated by Brushless (BL) DC motors. This yields the system's total DOF to be $18$ and control inputs $u\in\R^{12}$.
With different scenarios of foot contacts with the ground, we have a mixture of overactuated, fully-actuated, and underactuated domains (i.e., phases) for the dynamics. Futher, we can define the state space $\mathcal{X}=T\mathcal{Q}\subseteq \R^{2n}$ with the state vector $x^T = (q^T,\dot q^T)$, where $T\mathcal{Q}$ is the tangent bundle of the configuration space $\mathcal{Q}$. 

We now define the different modes of the quadrupedal dynamics, separated by discrete events. This fusion of continuous- and discrete-time dynamics yields a hybrid automaton model \cite{derIntro}. For more detailed definitions of hybrid modeling for bipedal robots, we refer the readers to \cite{Ames2013Humana}. 


\subsection{The continuous-time domain: constrained dynamics}
Given the floating base coordinates, we can derive the unconstrained dynamics, i.e. without any contact constraints, by the Euler-Lagrange equations as:
\begin{align*}
    D(q)\, \ddot q + H(q,\dot q) &= B u
\end{align*}
where $D(q)\in\R^{n\times n}$ is the mass-inertia matrix, $ H(q,\dot q)\in\R^n$ includes the Coriolis, centrifugal and gravity terms and $B(q)\in\R^{n\times m}$ is the actuation matrix and $u\in\R^m$ is the torque applied at joints with $m=12$.

Now consider $k\in\{1,2,3,4\}$ feet standing on the ground, which means $\bar k=4-k$ feet are swinging in the air. This creates a variety of contact scenarios, hence generates different types of quadrupedal behaviors (see \figref{fig:graph}). For each contact situation, we associate a \textit{continuous domain}:

\vspace{-3mm}
\small
\begin{align}
	\label{eq:domain}
	\mathcal{D}_v := \{ (x,u) | h_v(q)=\dot h_v(q,\dot q)=0, N_v \succeq 0, h_{\mathrm{s},v}(q)\succeq 0\}
\end{align}
\normalsize
where $v\in\{1,2,3...\}$ is the domain index and $h_v(q)\in\R^k$ is the height of all standing feet with ground reaction force $N_v(x,u)\in\R^k$. The height of the other feet, referred as the swing feet, is shown by $h_{\mathrm{s}, v}(q)\in\R^{\bar k}$. 
We then have the constrained dynamics for $\mathcal{D}_v$ as: %\cite{Murray1994mathematical} as:
\begin{align}\begin{cases}
D(q)\, \ddot q + H(q,\dot q) = B_v\, u + J_{v}^T(q)\, \lambda_v \\
J_v(q)\, \ddot q  + \dot J_v(q,\dot q)\, \dot q =0
\end{cases}
\label{eq:eom-general}
\end{align}
where $J_v(q):={\partial p_v(q)} / {\partial q}$ represents the Jacobian matrix of the Cartesian position of the standing feet $p_v(q)\in\R^{3k}$, with the corresponding constraint wrench $\lambda_v\in\R^{3k}$. 
% The first equation is considering ground forces as inputs and the second equation is treating the contacting as a holonomic constraint.
Note that the actuation matrix $B_v$ is domain dependent. This is because the double and triple support phases (\figref{fig:graph}) create closed-chain structures that induce redundancy in control and constraints. % that induces internal overactuation. 
This is an underdetermined problem which often appears in multi-contact locomotion \cite{zhaomulti} that yields nonunique controllers for $u$. Therefore, we manually turn off the rear standing leg's hip pitch motor for double support phase and turn off the diagonal standing legs' hip pitch motors and the other standing leg's hip roll motors for triple supporting phase. This implementation in return yields underactauted dynamics for the full system. Now we can convert the constrained EOM \eqref{eq:eom-general} into a controlled ODE:
\begin{align}
\label{eq:ode}
	\dot x = f_v(x) + g_v(x) u.
\end{align}
To track a given set of time-based trajectories $\mathcal{B}_v(t)$, which will be detailed in a later section, we deployed an \textit{input output feedback linearization} controller:
\begin{align}
\label{eq:io}
	u_{\mathrm{io}}(x,t) = \mathcal{A}(x) \big(  \mathcal{L}(x,t) - 2\varepsilon y(q,t) - \varepsilon^2 \dot y(q,\dot q, t)  \big).
\end{align}
with the outputs $y(q,t) = y_a(q)-\mathcal{B}_v(t)$ and $\varepsilon>0$. In this formulation, we chose the \textit{actual outputs} $y_a(q)$ as all of the actuated joints. The notations follow directly from Eq. (28) of \cite{Ames2013Humana}. The time-based controller has been justified for improved robustness over state-based methods both in theory \cite{DURUS_timedependent} and experiments \cite{ma2017bipedal}. As a result, \eqref{eq:io} forces the system to converge to a desired gait exponentially, that is, $y_a(q)\rightarrow \mathcal{B}_v(t)$. 
% Employing the feedback law in \eqref{eq:io} results in the following output dynamics:
The output dynamics become
\begin{align}
    \label{eq:ydyn}
	\ddot y = -2\varepsilon \dot y -\varepsilon^2 y
\end{align}
for which the origin $(y,\dot{y})=(0,0)$ is exponentially stable. 

\begin{figure}[!t]
\vspace{2mm}
	\begin{center}
		\includegraphics[width=0.9\columnwidth]{Figures/hybrid/directedGraph.png}
		\caption{The cyclic directed graph for the multi-domain hybrid dynamics of walking, ambling and trotting gaits. 
		The dashed lines represent a \textit{relabeling} map \cite{Ames2013Humana} that flips the left and right legs' contact attributes.
		% Refer to \figref{fig:gaits} for the full motion without relabelling map.
		% We only include half of periodic motion. Refer to \figref{fig:gaits} for the full motion. This is due to the left-right symmetry of the quadrupedal locomotion, one can flip the contact attributes on the left and right legs. This is referred to as the \textit{relabel mapping}, denoted by the dashed lines. 
		}
		\label{fig:graph}
	\end{center}
	\vspace{-5mm}
\end{figure} 

Prior to introducing the edges and the discrete dynamics, some assumptions are necessary to construct a feasible model both for computation and experiment:
\begin{itemize}
	\item There is no ground slippage. This is partially guaranteed by enforcing a friction cone condition. However, slipping locomotion has been observed on quadrupedal animals for energy efficiency \cite{gamus2013analysis, Maslipery}.
	
	% \item Only one foot can change its status at an instant time, meaning either one foot is leaving ground, or one foot is landing on the ground at one time.
	
	\item The ethology studies \cite{Muybridgeanimal} have observed a pattern of $4\times2$-domain\footnote{The term $m \times 2$ denotes a gait with $m$-domain. See \figref{fig:graph} for the directed graph of the gaits with $m$ domains. The second half of the motion is directly a left-right mirror (i.e., symmetry) of the gait. See \figref{fig:gaits} for the full motion with $m \times 2$ domains.}
	locomotion on quadrupedal animals, and the authors have investigated this modeling method in \cite{Hamed_Ma_Ames_Vision60}. But in this paper, we assume the \textit{stance leg transition domains ---one leg strikes while another leg lifts} are instantaneous and passive for walking and ambling. Hence $\mathbf{s}_1$ and $\mathbf{s}_2$ in \figref{fig:graph} become edges and we can have a $2\times 2$-domain behavior for \textit{walk} and \textit{amble}. 	
	But a $4\times 2$-domain model is still used for \textit{trot}.

\end{itemize}


\subsection{The discrete-time domain: impact and lift-off}
On the edge of $\mathcal{D}_v$ in \eqref{eq:domain}, one of the conditions reaches its bound. Thus we have two switching mechanisms:
\begin{itemize}
	%\item[$\mathcal{S}_1$.] 
	\item \textit{Lift off}: a standing foot of leg ${l_*}$ lifts off from the ground, meaning 
	$N_v^{l_*}(x,u) = 0$.
	
	%\item[$\mathcal{S}_2$.] 
	\item \textit{Impact}: a swing foot of leg $l_*$ impacts the ground, meaning $h_{s,v}^{l_*}(q) = 0$, $\dot h_{s,v}^{l_*}(q,\dot q) < 0$.
\end{itemize}
%
For \textit{lift off}, an identity map $x^+_{v+1} = x^-_{v}$ is sufficient to represent the transition from current to the next domain, where $x^-_{v}$ is the state at the end of the domain $\mathcal{D}_v$ and  $x^+_{v+1}$ is the state at the beginning of $\mathcal{D}_{v+1}$. However, the \textit{impact} shall cause a jump in the velocity terms. To describe this, we make use of a plastic impact model \cite{Grizzle2014Models},
\begin{align}
\label{eq:impact}
	\begin{bmatrix} D & -J_{v+1}^T\\ J_{v+1} &0 \end{bmatrix}
	\begin{bmatrix} \dot q^+_{v+1}\\ \Lambda \end{bmatrix}
	= 
	\begin{bmatrix} D \dot q^-_v\\ 0  \end{bmatrix}
\end{align}
by using the conservation of momentum while satisfying the next domain's holonomic constraints.



\input{sections/opt}


==> sections/Bgaitgen.tex <==
%\subsection{Gait Synthesis}
\label{sec:gaitsyn}
The desired trajectory $\mb{y}_d(\tau(\mb{q}),\alpha)$ is given by a degree $N$ Bézier polynomial
\[\mb{y}_d^i(\tau) = \sum_{k=0}^{N}\alpha_k^i \frac{N!}{k!(M-k)!}\tau^k (1-\tau)^{M-k}, \quad i\in \{1,...,m\} \]
With the relative degree 2 output defined for the hybrid control system $\Sigma$, the zero dynamic surface is defined as:
\begin{equation*} \label{eq:zdsurface}
    \mathcal{Z}(\delta_{hip}^-,\delta_{hip}^+,\bs{\alpha}) = \{ \mb{x} \in \mathcal{X}  \big| \y(\mb{q}) = 0 \mbox{ and } L_\f \y(\mb{q},\dot{\mb{q}}) = 0 \} 
\end{equation*}

For underactuated systems, \cite[Thm. 2]{ames2014rapidly} proved that with sufficiently rapidly exponentially stabilizing outputs, an exponentially stable periodic orbit in zero dynamics surface is an exponentially stable periodic orbit for the full-order dynamics.  The goal of the gait optimization is to find a periodic gait in the zero dynamics surface. 

The gait optimization is then performed with a feedback linearizing control law
\begin{equation}
    \u(\mb{x}) = -\left(L_\g L_\f \y(\mb{x})\right)^{-1} \left(\frac{1}{\epsilon}K_D L_\f \y(\mb{x}) +\frac{1}{\epsilon^2}K_P \y(\mb{x}) + L^2_\f\y(\mb{x})\right)
\end{equation}
which results in rapidly exponentially stabilizing output dynamics as $\Ddot{\y} = -\frac{1}{\epsilon}K_D \dot{\y} -\frac{1}{\epsilon^2}K_P \y$.

The optimization is performed to find a periodic orbit on the two-dimensional zero dynamics submanifold of $\mathcal{X}$, i.e. to find the set of parameters $\delta_{hip}^-,\delta_{hip}^+,\bs{\alpha}$ for desired outputs such that 
\[ \Delta(\mb{x}^-) \in \mathcal{Z}(\delta_{hip}^-,\delta_{hip}^+,\bs{\alpha}) ,\quad  \forall \mb{x}^- \in \mathcal{S} \cap \mathcal{Z}(\delta_{hip}^-,\delta_{hip}^+,\bs{\alpha}) \tag{HZD}\]
under a list of physical constraints including foot clearance, torso moving range, friction cone constraints and actuation limits. 

The gait optimization is a nonlinear program (NLP) performed under a direct collocation framework \cite{hereid2017frost}:
\begin{align*}
    \mathcal{X}^*  = \operatorname*{argmin}_{\chi} \quad & \Phi(\mathcal{X})\\
    \textrm{s.t.   }& \text{HZD}\\
    &\text{physical constraints}\\
\end{align*}
where $\mathcal{X}$ is a set of parameters in the NLP including $\delta_{hip}^-,\delta_{hip}^+$, and $\bs{\alpha}$.

==> sections/Cconvergence.tex <==

\label{sec:convergence}
The recursive relationship is made explicit in the closed-form solution to \eqref{eqn:delta-CBF-QP} (suppressing dependence on $\mb{x}$):
\begin{align}
    \mb{k}' = \begin{cases} 
                \mb{k}_d - L_{\widehat{\mb{g}}} h^\dagger \left( L_{\widehat{\mb{f}}}h + L_{\widehat{\mb{g}}}h \mb{k}_D + \alpha(h) + \widehat{\delta} \right), &  L_{\widehat{\mb{f}}}h + L_{\widehat{\mb{g}}}h + \alpha(h) + \widehat{\delta} < 0, \\ 
                \mb{k}_d,  &  L_{\widehat{\mb{f}}}h + L_{\widehat{\mb{g}}}h  + \alpha(h) + \widehat{\delta} \geq 0, 
                \end{cases}
\end{align}

Assume loss is zero at each step and $\delta_i(x)$ can be fully captured by learning. Also assume barrier is active (for same x?)
\\
For i-th iteration, the constraints in \eqref{eqn:delta-CBF-QP} that is being enforced is
\[L_{\hat{\f}}h(\x) + L_{\hat{\g}}h(\x)\k_i(\x) + \delta_{i-1}(\x) \geq -\alpha(h(\x))\]
The explicit solution of the QP can be written as:
\[\k_i(\x) = \k_{d}(\x) - L_{\hat{\g}}h^\dagger(\x) (L_{\hat{\f}}h(\x) + L_{\hat{\g}}h(\x) \k_d(\x) +\alpha(h(\x)) +\delta_{i-1}(\x)  )\]
The true dynamics of $\Dot{h}(\x)$ is given by
\[\Dot{h}(\x) = L_{\f}h(\x) + L_{\g}h(\x)\k_i(\x) = L_{\hat{\f}}h(\x) + L_{\hat{\g}}h(\x)\k_i(\x) + \delta_{i}(\x)\]
where $\delta_i(\x)$ is true residual that is learned after the i-th experiment:
\begin{align}
    \delta_i(\x) = b(\x) + \mb{a}(\x)^T \k_i(\x) =: \Delta_i(\x) - \delta_{i-1}(\x)
\end{align}
In i+1 th iteration, the constraints in \eqref{eqn:delta-CBF-QP} that is being enforced is
\[L_{\hat{\f}}h(\x) + L_{\hat{\g}}h(\x)\k_{i+1}(\x) + \delta_{i}(\x) \geq -\alpha(h(\x))\]
The explicit solution of the QP can be written as:
\[\k_{i+1}(\x) = \k_{d}(\x) - L_{\hat{\g}}h^\dagger(\x) (L_{\hat{\f}}h(\x) + L_{\hat{\g}}h(\x) \k_d(\x) +\alpha(h(\x)) +\delta_{i}(\x)  )\]
Subs in $\delta_{i}(\x) $ results in
\begin{align}
    \k_{i+1}(\x) = \k_i(\x) - L_{\hat{\g}}h^\dagger(\x) \Delta_i(\x)
\end{align}
The true dynamics of $\Dot{h}$ is given by
\[\Dot{h} = L_{\f}h(\x) + L_{\g}h(\x)\k_{i+1}(\x) = L_{\hat{\f}}h(\x) + L_{\hat{\g}}h(\x)\k_{i+1}(\x) + \delta_{i+1}(\x)\]
Thus, the difference of residue between iterations is given by
\begin{align}
    \Delta_{i+1}(\x) &= \delta_{i+1}(\x)-\delta_{i}(\x)\\
    &= b(\x) + \mb{a}(\x)^T \k_{i+1}(\x) - \delta_{i}(\x)\\
    &= b(\x) + \mb{a}(\x)^T (\k_i(\x) - L_{\hat{\g}}h^\dagger (\x) \Delta_i(\x)) - (b(\x) + \mb{a}(\x)^T \k_i(\x))\\
    &= -\mb{a}(\x)^T L_{\hat{\g}}h^\dagger(\x) \Delta_{i}(\x)
\end{align}
% Thus, $\k_N(x) = \k_d(\x) - L_{\hat{\g}}h^\dagger(\x) \sum_{i=0}^N \Delta_{i}(\x)$. 
% By Leibniz’s theorem, the alternating series $\sum_{i=0}^\infty \Delta_{i}(\x)$ converges
If $\| \mb{a}(\x) \|< (1-\epsilon)\| L_{\hat{\g}}h(\x)\|$ for some small $\epsilon >0$, then the residual is converging by Cauchy-Schwartz inequality and Leibniz’s theorem.

